Nebular phase properties of supernova Ibc from He-star explosions

Following our recent work on Type II supernovae (SNe), we present a set of 1D nonlocal thermodynamic equilibrium radiative transfer calculations for nebular-phase Type Ibc SNe starting from state-of-the-art explosion models with detailed nucleosynthesis. Our grid of progenitor models is derived from He stars that were subsequently evolved under the influence of wind mass loss. These He stars, which most likely form through binary mass exchange, synthesize less oxygen than their single-star counterparts with the same zero-age main sequence (ZAMS) mass. This reduction is greater in He-star models evolved with an enhanced mass loss rate. We obtain a wide range of spectral properties at 200d. In models from He stars with an initial mass >6Msun, the [OI] 6300, 6364 is of comparable or greater strength than [CaII] 7291,7323 -- the strength of [OI] 6300, 6364 increases with He-star initial mass. In contrast, models from lower mass He stars exhibit a weak [OI] 6300, 6364, strong [CaII] 7291,7323, but also strong NII lines and FeII emission below 5500A. The ejecta density, modulated by the ejecta mass, the explosion energy, and clumping, has a critical impact on the gas ionization, line cooling, and the spectral properties. FeII dominates the emission below 5500A and is stronger at earlier nebular epochs. It ebbs as the SN ages, while the fractional flux in [OI] 6300, 6364 and [CaII] 7291,7323 increases, with a similar rate, as the ejecta recombine. Although the results depend on the adopted wind mass loss rate and pre-SN mass, we find that He stars of 6-8Msun initially (ZAMS mass of 23-28Msun) match adequately the properties of standard SNe Ibc. Our results for less massive He stars are more perplexing, since the predicted spectra are not seen in nature. They may be missed by current surveys or associated with Type Ibn SNe in which interaction dominates over decay power. [Abridged]

==> model_composition_table.tex <==
\begin{table*}
    \caption{Ejecta model properties from \citet{ertl_ibc_20} -- see also Table~\ref{tab_prog_bis} and \ref{tab_ertliron}.
\label{tab_prog}
}
\begin{center}
\begin{tabular}{l@{\hspace{2mm}}|c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}}
\hline
Model  &  $M_{\rm preSN}$  & $M_{\rm ej}$  &     $E_{\rm kin}$   & $V_m$   &  \iso{4}He & \iso{12}C   & \iso{14}N  & \iso{16}O &  \iso{24}Mg &  \iso{28}Si &  \iso{40}Ca &  \iso{56}Ni$_{t=0}$ & $M_{\rm sh}$ & $V_{{\rm max},\nifs}$ \\
       &     [\msun] & [\msun]   &        [foe]    & [\kms]    &    [\msun] & [\msun] & [\msun] & [\msun] & [\msun] & [\msun] & [\msun] & [\msun] & [\msun] & [\kms] \\
\hline
%  Model     MpreSN     Mej        Ekin            Vm           he4            c12           n14           o16          mg24          si28          ca40          ni56    Msh    Vmax_ni56
   he2p6      & 2.15 &   0.79  &     0.13   &      4134   &      0.71    &      0.02  &   4.78(-3)   &   2.28(-2)   &   1.58(-3)   &   3.35(-3)   &   2.40(-4)   &   1.22(-2)  & 0.29 &  2697   \\
   he2p9      & 2.37 &   0.93  &     0.37   &      6336   &      0.77    &      0.04  &   5.15(-3)   &   5.03(-2)   &   3.82(-3)   &   1.01(-2)   &   5.62(-4)   &   2.32(-2)  & 0.38 &  4353   \\
   he3p3      & 2.67 &   1.20  &     0.55   &      6777   &      0.84    &      0.06  &   6.21(-3)   &   1.51(-1)   &   1.75(-2)   &   2.76(-2)   &   1.00(-3)   &   4.00(-2)  & 0.43 &  3712   \\
   he3p5      & 2.81 &   1.27  &     0.41   &      5704   &      0.87    &      0.07  &   6.31(-3)   &   1.72(-1)   &   1.60(-2)   &   2.13(-2)   &   7.34(-4)   &   2.92(-2)  & 0.49 &  3121   \\
   he4p0      & 3.16 &   1.62  &     0.63   &      6272   &      0.92    &      0.10  &   6.46(-3)   &   3.10(-1)   &   2.98(-2)   &   4.70(-2)   &   1.35(-3)   &   4.45(-2)  & 0.82 &  3974   \\
   he4p5L     & 3.49 &   1.89  &     0.54   &      5348   &      0.95    &      0.13  &   6.55(-3)   &   4.29(-1)   &   4.00(-2)   &   4.90(-2)   &   1.73(-3)   &   8.22(-2)  & 1.14 &  3532   \\
   he4p5      & 3.49 &   1.89  &     1.17   &      7884   &      0.95    &      0.13  &   6.52(-3)   &   4.19(-1)   &   3.73(-2)   &   6.14(-2)   &   2.40(-3)   &   8.59(-2)  & 1.14 &  5588   \\
   he4p5H     & 3.49 &   1.89  &     2.44   &     11400   &      0.97    &      0.12  &   6.38(-3)   &   3.96(-1)   &   3.55(-2)   &   7.86(-2)   &   3.33(-3)   &   9.03(-2)  & 1.14 &  8369   \\
   he5p0      & 3.81 &   2.21  &     1.51   &      8286   &      0.97    &      0.15  &   6.60(-3)   &   5.92(-1)   &   5.20(-2)   &   5.55(-2)   &   2.26(-3)   &   9.77(-2)  & 1.43 &  6164   \\
   he6p0      & 4.44 &   2.82  &     1.10   &      6269   &      0.95    &      0.25  &   6.20(-3)   &   9.74(-1)   &   1.01(-1)   &   5.88(-2)   &   2.12(-3)   &   7.04(-2)  & 2.16 &  4990   \\
   he7p0      & 5.04 &   3.33  &     1.38   &      6456   &      0.90    &      0.39  &   5.42(-3)   &   1.29       &   1.07(-1)   &   9.47(-2)   &   3.42(-3)   &   1.02(-1)  & 2.77 &  5356   \\
   he8p0      & 5.63 &   3.95  &     0.71   &      4251   &      0.84    &      0.49  &   5.17(-3)   &   1.71       &   1.10(-1)   &   4.89(-2)   &   2.00(-3)   &   5.46(-2)  & 3.40 &  3435   \\
   he12p0     & 7.24 &   5.32  &     0.81   &      3911   &      0.23    &      1.00  &   1.42(-4)   &   3.03       &   8.73(-2)   &   7.41(-2)   &   3.42(-3)   &   7.90(-2)  & 3.60 &  2531   \\
\hline
   he5p0x1p5    & 3.43  &  1.85  &   1.59   &      9299   &      0.86    &      0.16  &   6.18(-3)   &   4.22(-1)   &   3.27(-2)   &   6.34(-2)   &   2.74(-3)   &   1.11(-1)  & 1.12 &   6758  \\
   he6p0x1p5    & 3.96  &  2.32  &   1.57   &      8237   &      0.83    &      0.27  &   5.68(-3)   &   6.80(-1)   &   4.76(-2)   &   6.31(-2)   &   3.03(-3)   &   1.23(-1)  & 1.25 &   5787  \\
%  he7p0x1p5    & 4.45  &  2.84  &   1.46   &      7203   &      0.76    &      0.42  &   3.48(-3)   &   9.29(-1)   &   5.84(-2)   &   7.44(-2)   &   3.37(-3)   &   1.99(-1)  & 1.69 &         \\
   he8p0x1p5    & 4.92  &  3.26  &   1.49   &      6776   &      0.64    &      0.56  &   6.14(-4)   &   1.28       &   9.73(-2)   &   6.75(-2)   &   2.74(-3)   &   1.06(-1)  & 2.05 &   5096  \\
   he9p0x1p5    & 4.87  &  3.13  &   1.03   &      5743   &      0.26    &      0.62  &   1.55(-5)   &   1.49       &   9.36(-2)   &   8.39(-2)   &   3.58(-3)   &   1.21(-1)  & 2.07 &   4222  \\
   he10p0x1p5   & 4.96  &  3.20  &   1.22   &      6192   &      0.18    &      0.67  &   1.20(-5)   &   1.65       &   9.07(-2)   &   8.89(-2)   &   3.56(-3)   &   9.92(-2)  & 2.00 &   4465  \\
   he11p0x1p5   & 5.19  &  3.44  &   1.11   &      5705   &      0.20    &      0.76  &   4.24(-5)   &   1.78       &   7.16(-2)   &   6.26(-2)   &   2.72(-3)   &   4.26(-2)  & 2.13 &   4015  \\
   he12p0x1p5   & 5.43  &  3.71  &   0.97   &      5132   &      0.23    &      0.79  &   5.00(-5)   &   1.89       &   7.48(-2)   &   7.22(-2)   &   3.25(-3)   &   8.80(-2)  & 2.36 &   3561  \\
   he13p0x1p5   & 5.64  &  3.99  &     1.31   &      5736   &      0.24    &      0.82  &   7.19(-5)   &   2.04       &   7.38(-2)   &   8.26(-2)   &   3.78(-3)   &   1.28(-1)  & 2.60 &   4179  \\
\hline
   he10p0x2p0  &  3.98  & 2.22  &     1.23   &      7446   &      0.15    &      0.57  &   5.53(-6)  &   9.31(-1)    &   5.52(-2)   &   6.92(-2)   &   2.94(-3)   &   1.16(-1)  & 1.29 &  5233 \\
\hline
\end{tabular}
\end{center}
    {\bf Notes:} The table columns correspond to the preSN mass, the ejecta mass, the ejecta kinetic energy (1 foe $\equiv 10^{51}$\,erg), the mean expansion rate $V_{\rm m} \equiv \sqrt{2E_{\rm kin}/M_{\rm ej}}$, the cumulative yields of \iso{4}He, \iso{12}C, \iso{14}N, \iso{16}O, \iso{24}Mg, \iso{28}Si, \iso{40}Ca, and \nifs\ prior to decay. The last two columns give the Lagrangian mass $M_{\rm sh}$ adopted for the shell shuffling (see Sect.~\ref{sect_prep}), as well as the ejecta velocity that bounds 99\% of the total \nifs\ mass in the corresponding model (this value corresponds roughly to the velocity at the  Lagrangian mass $M_{\rm sh}$). All \nifs\ masses used here were taken from the \kepler\ approximation to the \photb\ neutrino simulation, and are between the best guess (\nifs+``Tr'') and generous upper bounds ($3/4 \times$(\nifs\ + ``Tr''+ $\alpha$)) defined by \citet[see also Table~\ref{tab_ertliron}]{ertl_ibc_20}.
\end{table*}

